New Choice for Small Universal Devices: Symport/Antiport P Systems

Symport/antiport P systems provide a very simple machinery inspired by corresponding operations in the living cell. It turns out that systems of small descriptional complexity are needed to achieve the universality by these systems. This makes them a good candidate for small universal devices replacing register machines for different simulations, especially when a simulating parallel machinery is involved. This article contains survey of these systems and presents different trade-offs between parameters.

==> eptcsdata.tex <==
\providecommand{\eid}{23}

